Artefact removal in ground truth and noise model deficient sub-cellular nanoscopy images using auto-encoder deep learning

Image denoising or artefact removal using deep learning is possible in the availability of supervised training dataset acquired in real experiments or synthesized using known noise models. Neither of the conditions can be fulfilled for nanoscopy (super-resolution optical microscopy) images that are generated from microscopy videos through statistical analysis techniques. Due to several physical constraints, supervised dataset cannot be measured. Due to non-linear spatio-temporal mixing of data and valuable statistics of fluctuations from fluorescent molecules which compete with noise statistics, noise or artefact models in nanoscopy images cannot be explicitly learnt. Therefore, such problem poses unprecedented challenges to deep learning. Here, we propose a robust and versatile simulation-supervised training approach of deep learning auto-encoder architectures for the highly challenging nanoscopy images of sub-cellular structures inside biological samples. We show the proof of concept for one nanoscopy method and investigate the scope of generalizability across structures, noise models, and nanoscopy algorithms not included during simulation-supervised training. We also investigate a variety of loss functions and learning models and discuss the limitation of existing performance metrics for nanoscopy images. We generate valuable insights for this highly challenging and unsolved problem in nanoscopy, and set the foundation for application of deep learning problems in nanoscopy for life sciences.

==> MUSICAL artifact removal/latexmkrc <==
## Sometimes when the references is very near the end of a page/column, latexmk fails to recognise when bibtex needs to be run. This rule forces bibtex to be run everytime.
$pdflatex = 'pdflatex --shell-escape %O %S; bibtex %R';



###############################
# Post processing of pdf file #
###############################

# assume the jobname is 'output' for Overleaf v2
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    my $QPDF = "/usr/bin/qpdf";
    return if ! -x $QPDF; # check that qpdf exists
    my $status = system($QPDF, "--linearize", "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
	system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
        $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
	system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
	if (-e $rtex_file) {
		do_knitr($rtex_file);
	}
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
	# change directory for a limited scope
	my $orig_dir = cwd();
	my $subdir = dirname($target);
	chdir($subdir);
	# run chktex on main file
	$status = system(
    "/usr/bin/run-chktex.sh",
    $orig_dir,
    $file
  );
	# go back to original directory
	chdir($orig_dir);

	# in VALIDATE mode we always exit after running chktex
	# otherwise we exit if EXIT_ON_ERROR is set

	if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
	    # chktex doesn't let us access the error info via exit status
	    # so look through the output
	    open(my $fh, "<", "output.chktex");
	    my $errors = 0;
	    {
		local $/ = "\n";
		while(<$fh>) {
		    if (/^\S+:\d+:\d+: Error:/) {
			$errors++;
			print;
		    }
		}
	    }
	    close($fh);
	    exit(1) if $errors > 0;
	    exit(0) if $ENV{'CHKTEX_VALIDATE'};
	}
    }
}

==> MUSICAL artifact removal/table_expt.tex <==

\begin{table}[b]
    \centering
    \begin{tabular}{|p{2 cm}|p{1.5 cm}|p{4cm}|p{3 cm}|c|}
    \hline
        Sample & Data source & Microscope and dye parameters & Imaging conditions & SBR \\
    \hline
    \hline
        Actin filaments & Example xx of \cite{agarwal2016multiple} & Total internal reflection microscope, NA 1.49, sCMOS camera, pixel size 65 nm, dye ATTO 647 emission wavelength 610 nm  & Exposure time xx ms, Acquisition rate xx ms, Number of frames used xx & xx \\
    \hline
         Liposomes in agarose & Example xx of \cite{arxiv Fl. rev.} & \remark{Sebastian}{help me complete}  & Exposure time xx ms, Acquisition rate xx ms, Number of frames used xx & xx \\
    \hline
         Mitochondria in living cell & Example xx of \cite{imageJ site or otherwise} & \remark{Sebastian}{help me complete}  & Exposure time xx ms, Acquisition rate xx ms, Number of frames used xx & xx \\
    \hline
         Microtubules in fixed cell & Example xx of \cite{debias} & \remark{Sebastian}{help me complete}  & Exposure time xx ms, Acquisition rate xx ms, Number of frames used xx & xx \\
    \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:expt}
\end{table}


==> MUSICAL artifact removal/table_psnr.tex <==
\begin{table}[b]
\caption{Quantitative analysis in terms of PSNR for different combinations of models and loss functions. The method with the best PSNR value is highlighted in bold. Further, the three methods M1-M3 used for qualitative comparison are indicated in underline.}
\small
{
    % \centering
    \begin{tabular}{|l||c|c|c|c|c|c|c||c|}
    \hline
     & \multicolumn{7}{c||}{\textbf{Loss functions}}     &  \\ 
    \cline{2-8}\vspace{-2 mm}
    & \textbf{L2} & \textbf{L1} &
    \textbf{SSIM} & \textbf{MS-SSIM} &
    \textbf{VGG} & \textbf{MS-SSIM} &
    \textbf{SSIM} & \textbf{Best loss}\\
    \textbf{Model} &&&&&& $+$ \textbf{L1} & $+$ \textbf{L1} & \textbf{function}\\
    \hline\hline
    \multicolumn{9}{|c|}{Actin filaments}\\
    \hline
    UNet(R-34) & 38.27          & 37.64 & 35.89 & 36.27 & 37.69 & 37.21 & 37.11 & L2 \\
    UNet(R-50) & \underline{37.94}          & 36.61 & 37.58 & 36.74 & \underline{38.60} & \underline{37.43} & 37.99 & VGG \\
    FPN(R-34)  & \textbf{38.71} & 37.26 & 36.76 & 37.31 & {35.28} & 36.93 & 36.25 & L2 \\
    %FPN(R-50)  & 35.26          & 36.99 & 35.36 & 37.13 & 36.83 & 37.07 & 36.76 & MS-SSIM \\
    \hline\vspace{-2mm}
    \textbf{Best} & FPN & UNet & UNet & FPN & UNet & UNet & UNet & \\
    \textbf{Model} & R-34 & R-34 & R-50 & R-34 & R-50 & R-50 & R-50 & \\
    \hline\hline
    \multicolumn{9}{|c|}{Vesicles}\\
    \hline
    UNet(R-34) & 39.29 & 38.96 & 38.66 & 37.62 & 39.78          & 37.89 & 38.63 & VGG \\
    UNet(R-50) & \underline{39.64} & 39.18 & 38.62 & 37.28 & \underline{\textbf{39.91}} & \underline{38.31} & 39.61 & VGG \\
    FPN(R-34)  & 38.75 & 37.62 & 37.36 & 37.78 & {35.36}          & 37.87 & 37.57 & L2 \\
    %FPN(R-50)  & {35.36} & 36.76 & 37.34 & 36.84 & 38.18          & 36.99 & 39.00 & SSIM + L1 \\
    \hline\vspace{-2mm}
    \textbf{Best} & UNet & UNet & UNet & FPN & UNet & UNet & UNet & \\
    \textbf{Model} & R-50 & R-50 & R-34 & R-34 & R-50 & R-50 & R-50 & \\
    \hline\hline
    \multicolumn{9}{|c|}{Mitochondria}\\
    \hline
    UNet(R-34) & 38.13 & 37.19 & 38.05 & {35.46} & 38.97          & 38.63 & 38.21 & VGG \\
    UNet(R-50) & \underline{36.59} & 36.73 & 39.20 & 38.69 & \underline{\textbf{40.36}} & \underline{37.42} & 39.98 & VGG \\
    FPN(R-34)  & 40.05 & 38.18 & 38.21 & 37.35 & 37.00          & 38.87 & 39.97 & L2 \\
    %FPN(R-50)  & 37.01 & 38.64 & 35.93 & 37.45 & 37.94          & 38.41 & 36.17 & L1 \\
    \hline\vspace{-2mm}
    \textbf{Best} & FPN & FPN & UNet & UNet & UNet & FPN & UNet &  \\
    \textbf{Model} & R-34 & R-34 & R-50 & R-50 & R-50 & R-34 & R-50 &  \\
    \hline
    \end{tabular}}
\label{tab:metric-values}
\end{table}

==> MUSICAL artifact removal/table_sim.tex <==

\begin{table}
\small
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Parameter}                & \textbf{Value}     & \textbf{Parameter}                 & \textbf{Value}             \\ \hline
Numerical Aperture (NA)           & {[}1.2, 1.49{]}    & Z coordinate range                 & {[}200, 1200{]} nm         \\ \hline
Magnification                     & 1                  & X and Y coordinate range           & {[}-2500, 2500{]} nm       \\ \hline
Wavelength                        & 660 nm             & \begin{tabular}[c]{@{}c@{}}Maximum length of a single strand \\ (mitochondria and actins)\end{tabular} & 5000 nm \\ \hline
Pixel Size                        &  \{65, 80, 108, 120\} nm &  \begin{tabular}[c]{@{}c@{}}Degree of the spline curve\\ (mitochondria and actins)\end{tabular} & {[}3, 6{]} \\ \hline
Low-Res Image Size                & 70 px              & Diameter of a single mitochondrion & 300 nm                     \\ \hline
No. of frames per stack           & 200                & Radius of a single vesicle         & {[}25, 500{]} nm           \\ \hline
$T_{off}$                         & {[}1, 20{]} frames & $\rho_{e}^{actin}$                 & 0.1 nm\textsuperscript{-1} \\ \hline
$T_{on}$                          & {[}1, 5{]} frames  & $\rho_{e}^{mitochondrion}$ & 0.5x10\textsuperscript{-3} nm\textsuperscript{-2} \\ \hline
Actin count (in a single image)   & {[}3, 10{]}        & $\rho_{e}^{vesicle}$               & 2 (\textcolor{green}{confirm unit})           \\ \hline
\begin{tabular}[c]{@{}c@{}}Mitochondrion count  \\ (in a single image) \end{tabular} &  {[}1, 4{]} &  \begin{tabular}[c]{@{}c@{}}Signal-to-Background Ratio (SBR)\\ for Poisson noise\end{tabular} &  3 \\ \hline
Vesicle Count (in a single image) & {[}10, 30{]}       & Camera noise (b)                   & 100                        \\ \hline
\end{tabular}
\caption{Simulation Parameters used for generating the dataset. Square brackets denote the range of values out of which one was chosen at random during the simulation. For NA and the radius of a single vesicle, a real number was randomly chosen within the specified range. For the rest of the parameters (excluding X, Y, and Z coordinate ranges), an integer value was chosen within the range. \newline
$T_{off}$ = Average no. of frames for which the emitters were turned off \newline
$T_{on}$ = Average no. of frames for which the emitters were turned on \newline
$\rho_{e}$ = Emitter density}
\label{tab:sim-params}
\end{table}

==> latexmkrc <==
## Sometimes when the references is very near the end of a page/column, latexmk fails to recognise when bibtex needs to be run. This rule forces bibtex to be run everytime.
$pdflatex = 'pdflatex --shell-escape %O %S; bibtex %R';



###############################
# Post processing of pdf file #
###############################

# assume the jobname is 'output' for Overleaf v2
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    my $QPDF = "/usr/bin/qpdf";
    return if ! -x $QPDF; # check that qpdf exists
    my $status = system($QPDF, "--linearize", "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
	system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
        $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
	system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
	if (-e $rtex_file) {
		do_knitr($rtex_file);
	}
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
	# change directory for a limited scope
	my $orig_dir = cwd();
	my $subdir = dirname($target);
	chdir($subdir);
	# run chktex on main file
	$status = system(
    "/usr/bin/run-chktex.sh",
    $orig_dir,
    $file
  );
	# go back to original directory
	chdir($orig_dir);

	# in VALIDATE mode we always exit after running chktex
	# otherwise we exit if EXIT_ON_ERROR is set

	if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
	    # chktex doesn't let us access the error info via exit status
	    # so look through the output
	    open(my $fh, "<", "output.chktex");
	    my $errors = 0;
	    {
		local $/ = "\n";
		while(<$fh>) {
		    if (/^\S+:\d+:\d+: Error:/) {
			$errors++;
			print;
		    }
		}
	    }
	    close($fh);
	    exit(1) if $errors > 0;
	    exit(0) if $ENV{'CHKTEX_VALIDATE'};
	}
    }
}

==> table_expt.tex <==

\begin{table}[b]
    \centering
    \begin{tabular}{|p{2 cm}|p{1.5 cm}|p{4cm}|p{3 cm}|c|}
    \hline
        Sample & Data source & Microscope and dye parameters & Imaging conditions & SBR \\
    \hline
    \hline
        Actin filaments & Example xx of \cite{agarwal2016multiple} & Total internal reflection microscope, NA 1.49, sCMOS camera, pixel size 65 nm, dye ATTO 647 emission wavelength 610 nm  & Exposure time xx ms, Acquisition rate xx ms, Number of frames used xx & xx \\
    \hline
         Liposomes in agarose & Example xx of \cite{arxiv Fl. rev.} & \remark{Sebastian}{help me complete}  & Exposure time xx ms, Acquisition rate xx ms, Number of frames used xx & xx \\
    \hline
         Mitochondria in living cell & Example xx of \cite{imageJ site or otherwise} & \remark{Sebastian}{help me complete}  & Exposure time xx ms, Acquisition rate xx ms, Number of frames used xx & xx \\
    \hline
         Microtubules in fixed cell & Example xx of \cite{debias} & \remark{Sebastian}{help me complete}  & Exposure time xx ms, Acquisition rate xx ms, Number of frames used xx & xx \\
    \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:expt}
\end{table}


==> table_sim.tex <==

\begin{table}
\small
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Parameter}                & \textbf{Value}     & \textbf{Parameter}                 & \textbf{Value}             \\ \hline
Numerical Aperture (NA)           & {[}1.2, 1.49{]}    & Z coordinate range                 & {[}200, 1200{]} nm         \\ \hline
Magnification                     & 1                  & X and Y coordinate range           & {[}-2500, 2500{]} nm       \\ \hline
Wavelength                        & 660 nm             & \begin{tabular}[c]{@{}c@{}}Maximum length of a single strand \\ (mitochondria and actins)\end{tabular} & 5000 nm \\ \hline
Pixel Size                        &  \{65, 80, 108, 120\} nm &  \begin{tabular}[c]{@{}c@{}}Degree of the spline curve\\ (mitochondria and actins)\end{tabular} & {[}3, 6{]} \\ \hline
Low-Res Image Size                & 70 px              & Diameter of a single mitochondrion & 300 nm                     \\ \hline
No. of frames per stack           & 200                & Radius of a single vesicle         & {[}25, 500{]} nm           \\ \hline
$T_{off}$                         & {[}1, 20{]} frames & $\rho_{e}^{actin}$                 & 0.1 nm\textsuperscript{-1} \\ \hline
$T_{on}$                          & {[}1, 5{]} frames  & $\rho_{e}^{mitochondrion}$ & 0.5x10\textsuperscript{-3} nm\textsuperscript{-2} \\ \hline
Actin count (in a single image)   & {[}3, 10{]}        & $\rho_{e}^{vesicle}$               & 2 (\textcolor{green}{confirm unit})           \\ \hline
\begin{tabular}[c]{@{}c@{}}Mitochondrion count  \\ (in a single image) \end{tabular} &  {[}1, 4{]} &  \begin{tabular}[c]{@{}c@{}}Signal-to-Background Ratio (SBR)\\ for Poisson noise\end{tabular} &  3 \\ \hline
Vesicle Count (in a single image) & {[}10, 30{]}       & Camera noise (b)                   & 100                        \\ \hline
\end{tabular}
\caption{Simulation Parameters used for generating the dataset. Square brackets denote the range of values out of which one was chosen at random during the simulation. For NA and the radius of a single vesicle, a real number was randomly chosen within the specified range. For the rest of the parameters (excluding X, Y, and Z coordinate ranges), an integer value was chosen within the range. \newline
$T_{off}$ = Average no. of frames for which the emitters were turned off \newline
$T_{on}$ = Average no. of frames for which the emitters were turned on \newline
$\rho_{e}$ = Emitter density}
\label{tab:sim-params}
\end{table}
